Enhancing respiratory comfort with fan respirators: computational analysis of carbon dioxide reduction, temperature regulation, and humidity control

Respirators provide protection from inhalation exposure to dangerous substances, such as chemicals and infectious particles, including SARS-Covid-laden droplets and aerosols. However, they are prone to exposure to stale air as the masks creat a microclimate influenced by the exhaled air. As a result, exhaled air from the lungs accumulating in the mask produce a warm and humid environment that has a high concentration of carbon dioxide (CO2), unsuitable for re-inhalation. Fans are a favourable option for respirators to ventilate the mask and remove the stale air. This study utilized computational fluid dynamics simulation consisting of a hybrid Reynolds-averaged Navier-Stokes (RANS)-large eddy simulation (LES) turbulence method to compare the inhalation flow properties for different fan locations (bottom, top, and side) with regular respirator breathing. Three mask positions, top, side, and bottom, were evaluated under two breathing cycles (approximately 9.65s of breathing time). The results demonstrated that adding a fan respirator significantly decreased internal mask temperature, humidity, and CO2 concentration. The average CO2 concentration decreased by 87%, 67% and 73% for locations bottom, top and side respectively. Whilst the top and side fan locations enhanced the removal of the exhaled gas mixture, the bottom-fan respirator was more efficient in removing the nostril jet gas mixture and therefore provided the least barrier to respiratory function. The results provide valuable insights into the benefits of fan respirators for long-term use for reducing CO2 concentration, mask temperature, and humidity, improving wearer safety and comfort in hazardous environments, especially during the COVID-19 pandemic.

==> figs.tex <==




